ThreadBench: Benchmarking Realism in Agentic Simulation of Real-world Discussions

LLM agents are increasingly used to simulate real-world interactions, but it remains unclear whether simulated behaviors preserve the content patterns and interaction dynamics of real human behaviors. Existing evaluations often focus on individual comments or task performance, rather than whether simulated behaviors match human behavior at thread level. In this paper, we use Reddit discussions as a concrete testbed for real-world social simulation. Reddit provides public, topic-grounded, multi-party interactions with diverse opinions, experiences, and interaction patterns, making it a useful setting for evaluating whether LLM agents reproduce the distributional and structural properties of real online discussions. We introduce ThreadBench, a benchmark for Reddit discussion simulation built from 9,817 real Reddit threads spanning 8 diverse domains and 116 subdomains. ThreadBench uses statistical analyses to compare generated and real discussions across 12 metrics grouped in 4 families: uniformity, expression, tone, and interaction. We further develop Thread-Prompt-based Discussion Generation (ThreadPDG), a Planner-Writer framework that learns how a real discussion grows. The Planner produces thread- and comment-level plans from a real seed discussion, and the Writer generates comments from these plans. For each seed, we generate multiple candidate threads and combine their best branches using thread-level statistics. Across all domains and multiple LLMs, ThreadPDG achieves ThreadBench pass rates of 58-100%, compared with 0-17% for the baselines. Human evaluation with 436 annotators further shows that ThreadPDG is not distinguished from real discussions in 78.7% of pairs, outperforming existing simulation methods.

==> sections/4-method.tex <==



\section{Prompt-based Calibration Study}
\label{sec:method}



We study prompt-based calibration as a validation-guided prompt revision process. 
At each step, MiroBench compares simulated discussions with real validation discussions, identifies metric gaps, and uses these diagnostics to guide candidate prompt revisions. 
Each candidate prompt is tested by running a fresh simulation, and the candidate that best reduces the validation discrepancy is kept. 
The final revised prompt is then evaluated on the held-out test split.



\subsection{Calibration Setup}
For each domain, let $\mathcal{D}^{real}_{train}$, $\mathcal{D}^{real}_{val}$, and $\mathcal{D}^{real}_{test}$ denote the real train, validation, and test splits. 
The train split provides qualitative examples of real Reddit discussions. 
The validation split is used to select prompt changes during calibration. 
The test split is held out for before/after calibration. For each discussion thread $t$, MiroBench computes a vector of thread-level metric scores:
$
m(t) = \{m_1(t), m_2(t), \ldots, m_K(t)\}.
$
For each metric $m_k$, the real validation threads define a reference distribution $R_k$, and the simulated threads generated under a prompt revision $\theta$ define a generated distribution $G_k(\theta)$. The prompt revision is restricted to two editable fields:
$
\theta = \{\theta^{persona}, \theta^{style}\},
$
where $\theta^{persona}$ controls persona generation guidance and $\theta^{style}$ controls comment writing guidance. Persona guidance affects simulated users' background, product experience, confidence level, personal memories, and reasons for joining the discussion. Style guidance affects comment length, anecdote use, disagreement style, short replies, repeated phrasing, and reactions to earlier comments. 

\subsection{Calibration Objective}

We formulate prompt calibration as a distribution-matching problem. 
For each metric $m_k$, we define a discrepancy score between the real validation distribution $R_k$ and the generated distribution $G_k(\theta)$:
\[
d_k(\theta)
=
\lambda_W \widetilde{W}_k(\theta)
+
\lambda_C |\Delta_k(\theta)|
+
\lambda_P P_k(\theta).
\]
Here, $\widetilde{W}_k(\theta)$ is the normalized Wasserstein distance, $|\Delta_k(\theta)|$ is the absolute Cliff's delta, and $P_k(\theta)$ is a penalty based on Mann--Whitney U and Kolmogorov--Smirnov tests. Lower $d_k(\theta)$ means that the simulated distribution is closer to the real distribution for metric $m_k$.

At each iteration $i$ of block $b$, we select the candidate prompt by minimizing the following block-wise objective:
\[
\theta_i^\star
=
\arg\min_{\theta \in \Theta_{i,b}}
\left[
\sum_{k \in \mathcal{M}^{act}_b} w_k d_k(\theta)
+
\gamma
\sum_{k \in \mathcal{M}^{prot}_b}
\max \left(0, d_k(\theta) - d_k(\theta^{base}_b)\right)
\right],
\]
where $\theta^{base}_b$ is the cumulative prompt before block $b$ starts, and $\Theta_{i,b}=\{\theta^{cum}+\Delta\theta_{i,c}\}_{c=1}^{C}$ is the candidate prompt set at iteration $i$ of block $b$. 
The first term measures improvement on the current metric group, and the second term penalizes regressions on protected metrics. 
Within each block, we keep the best candidate prompt update as $\Delta\theta_b^\star$. 
After each block, we update the cumulative prompt as $\theta^{cum} \leftarrow \theta^{cum} + \Delta\theta_b^\star$, and the final prompt is the cumulative prompt after all blocks.

\subsection{Calibration Workflow}
\textbf{Candidate Generation}
We use a fixed 12-iteration calibration schedule divided into four groups of metrics, with three iterations per group. At iteration $i$ of block $b$, we first compute validation diagnostics:
\[
D_i =
\textsc{Diag}
\left(
S(\theta^{cum} + \Delta\theta_b^\star),
\mathcal{D}^{real}_{val},
\mathcal{M}^{act}_b
\right),
\]
where $S$ is the simulator, $\theta^{cum}$ is the cumulative prompt revision from previous blocks, and $\Delta\theta_b^\star$ is the best prompt update found so far in the current block. Candidate generation uses two LLM steps. 

1) At iteration $i$ of block $b$, the strategist LLM receives the tuple
\[
x^{strat}_{i,b}
=
\left(
D_i,\ 
g_b,\ 
H_b,\ 
E^{real}_{train},\ 
E^{sim}_{i}
\right),
\]
where $D_i$ denotes the current validation diagnostics, $g_b$ is the goal of block $b$, $H_b$ is the history of previous candidate results within the same block, $E^{real}_{train}$ is a small set of real discussion examples sampled from $\mathcal{D}^{real}_{train}$, and $E^{sim}_{i}$ is a small set of simulated examples generated by the current prompt. 
Given this input, the strategist proposes high-level directions for improving the current metric group:
$
\{r_{i,c}\}_{c=1}^{C}
=
\textsc{Strategist}(x^{strat}_{i,b}).
$

2) a materializer LLM turns each direction into concrete text for the two editable prompt fields:
\[
\Delta\theta_{i,c}
=
\textsc{Materializer}(r_{i,c})
=
\{\Delta\theta^{persona}_{i,c}, \Delta\theta^{style}_{i,c}\}.
\]

\textbf{Candidate Evaluation and Selection} Each candidate prompt update is added to the current cumulative prompt revision:
$
\theta_{i,c} = \theta^{cum} + \Delta\theta_{i,c}.
$
We then run a fresh simulation:
$
T_{i,c} = S(\theta_{i,c}),
$
and score the resulting threads with MiroBench. 
The candidate is evaluated by the block-level validation loss:
\[
s_{i,c}
=
\mathcal{L}_b
\left(
\theta_{i,c};
S,
\mathcal{D}^{real}_{val},
\mathcal{M}^{act}_b,
\mathcal{M}^{prot}_b,
\theta^{base}_b
\right).
\]

The best candidate at iteration $i$ is:
$
c^\star = \arg\min_{c \in \{1,\ldots,C\}} s_{i,c}.
$
If this candidate improves the best score found in the current block, we update the block-best prompt update:
$
(\Delta\theta_b^\star, s_b^\star)
\leftarrow
(\Delta\theta_{i,c^\star}, s_{i,c^\star}).
$

At the end of each block, the block-best prompt update is added to the cumulative prompt revision:
$
\theta^{cum} \leftarrow \theta^{cum} + \Delta\theta_b^\star.
$
The final prompt revision is therefore built as:
\[
\theta^{final}
=
\theta^{story}
+
\theta^{diversity}
+
\theta^{length}
+
\theta^{tone}.
\]
Earlier prompt changes are preserved, and later blocks append new guidance rather than replacing the whole prompt. The pseudo-code is shown in the Algorithm ~\ref{alg:prompt_calibration}

\textbf{Final Evaluation} After all 12 iterations, we run a fresh simulation using $\theta^{final}$. 
This simulation is compared against $\mathcal{D}^{real}_{test}$. We report the same before/after statistics used in the benchmark: MWU and KS $p$-value counts, Wasserstein distance, and absolute Cliff's delta. 
This separates prompt selection from final reporting and reduces the risk of overfitting to the validation split. 

\begin{algorithm}[t]
\caption{Prompt-based Calibration}
\label{alg:prompt_calibration}
\begin{algorithmic}[1]
\Require Simulator $S$, train split $\mathcal{D}^{real}_{train}$, validation split $\mathcal{D}^{real}_{val}$, block schedule $\mathcal{B}$, candidates per iteration $C$
\Ensure Calibrated prompt revision $\theta^{final}$

\State Initialize cumulative prompt revision $\theta^{cum} \leftarrow \emptyset$

\For{$b \in \mathcal{B}$}
    \State Get active and protected metrics $(\mathcal{M}^{act}_b, \mathcal{M}^{prot}_b) \leftarrow \Phi(b)$
    \State Set block base prompt revision $\theta^{base}_b \leftarrow \theta^{cum}$
    \State Initialize block-best prompt update and score $(\Delta\theta_b^\star, s_b^\star) \leftarrow (\emptyset, +\infty)$

    \For{$i = 1,\ldots,I_b$}
        \State Compute diagnostics:
        $
        D_i \leftarrow 
        \textsc{Diag}
        \left(
        S(\theta^{cum}+\Delta\theta_b^\star),
        \mathcal{D}^{real}_{val},
        \mathcal{M}^{act}_b
        \right)
        $

        \State Generate high-level directions:
        $
        \{r_{i,c}\}_{c=1}^{C}
        \leftarrow
        \textsc{Strategist}
        \left(
        D_i,
        b,
        \mathcal{D}^{real}_{train}
        \right)
        $

        \State Materialize prompt updates:
        $
        \{\Delta\theta_{i,c}\}_{c=1}^{C}
        \leftarrow
        \textsc{Materializer}
        \left(
        \{r_{i,c}\}_{c=1}^{C}
        \right)
        $

        \For{$c = 1,\ldots,C$}
            \State Apply candidate update $\theta_{i,c} \leftarrow \theta^{cum} + \Delta\theta_{i,c}$
            \State Evaluate candidate:
            $
            s_{i,c}
            \leftarrow
            \mathcal{L}_b
            \left(
            \theta_{i,c};
            S,
            \mathcal{D}^{real}_{val},
            \mathcal{M}^{act}_b,
            \mathcal{M}^{prot}_b,
            \theta^{base}_b
            \right)
            $
        \EndFor

        \State Select best candidate $c^\star \leftarrow \arg\min_{c \in \{1,\ldots,C\}} s_{i,c}$

        \If{$s_{i,c^\star} < s_b^\star$}
            \State Update block best $(\Delta\theta_b^\star, s_b^\star) \leftarrow (\Delta\theta_{i,c^\star}, s_{i,c^\star})$
        \EndIf
    \EndFor

    \State Update cumulative prompt revision $\theta^{cum} \leftarrow \theta^{cum} + \Delta\theta_b^\star$
\EndFor

\State $\theta^{final} \leftarrow \theta^{cum}$
\State \Return $\theta^{final}$
\end{algorithmic}
\end{algorithm}

==> sections/5-Results.tex <==
\section{Experiments and Results}
\label{sec:experiments_results}

\subsection{Baseline and Calibration Results on ThreadBench}
\label{sec:baseline_results}

\textbf{Baselines.}
We evaluate OASIS~\cite{yang2411oasis} and SynthPAI~\citep{yukhymenko2024synthetic} as uncalibrated discussion simulation baselines on ThreadBench.
OASIS represents an LLM-agent simulation setting where multiple agents interact to generate Reddit-like discussions.
SynthPAI uses a persona-based synthetic interaction setting where simulated users produce discussion content from generated profiles.
We also evaluate our PDG(\textbf{P}rompt-based \textbf{D}iscussion Generation) as detailed in Section~\ref{sec:method}.

% \begin{table*}[t]
% \centering
% \tiny
% \setlength{\tabcolsep}{2.0pt}
% \renewcommand{\arraystretch}{0.92}

% \caption{
% Distributional similarity between simulated and real discussions across
% methods, model families, and domains.
% For each metric, we report two-sided Mann--Whitney U (MWU) and
% Kolmogorov--Smirnov (KS) test $p$-values.
% Values with $p \geq 0.05$ are shown in bold.
% \textit{Non-rej.} denotes the percentage of the 24 tests
% (12 metrics $\times$ 2 tests) for which the null hypothesis of no
% distributional difference is not rejected.
% }
% \vspace{3pt}
% \label{tab:full_domain_metric_comparison}

% \resizebox{\textwidth}{!}{
% \begin{tabular}{
% lll
% *{12}{cc}
% c
% }
% \toprule

% \multirow{2}{*}{\textbf{Method}}
% & \multirow{2}{*}{\textbf{Model}}
% & \multirow{2}{*}{\textbf{Domain}}

% & \multicolumn{2}{c}{\textbf{Self-BLEU}}
% & \multicolumn{2}{c}{\textbf{Self-BERT}}
% & \multicolumn{2}{c}{\textbf{Sem. Cos.}}
% & \multicolumn{2}{c}{\textbf{Hard Dis.}}
% & \multicolumn{2}{c}{\textbf{Polite}}
% & \multicolumn{2}{c}{\textbf{Impolite}}
% & \multicolumn{2}{c}{\textbf{Neutral}}
% & \multicolumn{2}{c}{\textbf{Len. CV}}
% & \multicolumn{2}{c}{\textbf{Depth}}
% & \multicolumn{2}{c}{\textbf{Virality}}
% & \multicolumn{2}{c}{\textbf{Story}}
% & \multicolumn{2}{c}{\textbf{Emotion}}
% & \multirow{2}{*}{\shortstack{\textbf{Non-rej.}\\\textbf{(\%)}}}
% \\

% \cmidrule(lr){4-5}
% \cmidrule(lr){6-7}
% \cmidrule(lr){8-9}
% \cmidrule(lr){10-11}
% \cmidrule(lr){12-13}
% \cmidrule(lr){14-15}
% \cmidrule(lr){16-17}
% \cmidrule(lr){18-19}
% \cmidrule(lr){20-21}
% \cmidrule(lr){22-23}
% \cmidrule(lr){24-25}
% \cmidrule(lr){26-27}

% & & &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% MWU & KS &
% \\

% \midrule

% % =========================================================
% % OASIS — GPT-4o-mini
% % =========================================================
% \multirow{48}{*}{OASIS}
% & \multirow{12}{*}{gpt-4o-mini}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & Camera
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & Celebrity
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & Cellphone
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & Game
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & Headphones
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & Health Issue
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & Laptop
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & Movies
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & News
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & Sports
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% & & TV Series
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% \cmidrule(lr){2-28}

% % =========================================================
% % OASIS — GPT-5.4-mini
% % =========================================================
% & \multirow{12}{*}{gpt-5.4-mini}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % ... repeat 11 domains ...

% \cmidrule(lr){2-28}

% % =========================================================
% % OASIS — Gemini-2.5-Flash
% % =========================================================
% & \multirow{12}{*}{gemini-2.5-flash}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % ... repeat 11 domains ...

% \cmidrule(lr){2-28}

% % =========================================================
% % OASIS — DeepSeek-V4-Flash
% % =========================================================
% & \multirow{12}{*}{deepseek-v4-flash}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % ... repeat 11 domains ...

% \midrule

% % =========================================================
% % SynthPAI
% % Same 4 models × 12 domains
% % =========================================================

% \multirow{48}{*}{SynthPAI}
% & \multirow{12}{*}{gpt-4o-mini}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % ... repeat all 12 domains × 4 models ...

% \midrule

% % =========================================================
% % Ours
% % 4 single-family configs + 1 mixed config
% % =========================================================

% \multirow{60}{*}{\textbf{Ours}}
% & \multirow{12}{*}{gpt-4o-mini}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % ... repeat all 12 domains ...

% \cmidrule(lr){2-28}

% & \multirow{12}{*}{gpt-5.4-mini}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % ... repeat all 12 domains ...

% \cmidrule(lr){2-28}

% & \multirow{12}{*}{gemini-2.5-flash}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % ... repeat all 12 domains ...

% \cmidrule(lr){2-28}

% & \multirow{12}{*}{deepseek-v4-flash}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % ... repeat all 12 domains ...

% \cmidrule(lr){2-28}

% & \multirow{12}{*}{
% \shortstack[l]{
% mixed\\
% P: gpt-5.4-mini\\
% W: deepseek-v4-flash}}
% & Credit Card
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & --
% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

% % ... repeat all 12 domains ...

% \bottomrule
% \end{tabular}
% }
% \end{table*}

Table~\ref{tab:baseline_compact_pvalue_summary} summarizes the simulation-vs.-real statistical tests.
Each entry counts how many of the 12 core metrics are not statistically distinguishable from held-out real discussions at $p \geq 0.05$.
The uncalibrated OASIS baseline shows the largest mismatch: across all five domains, both MWU and KS counts are 0/12.
This means that every core metric remains statistically distinguishable from real Reddit discussions.
SynthPAI improves some MWU counts, especially in Cellphone and Camera, but its KS counts remain 0/12 across all domains.
This suggests that some rank-based differences are reduced, while the full distributional shapes remain far from real discussions.

Prompt-based calibration gives modest but broader gains.
Compared with OASIS, it improves MWU counts in four of the five domains, reaching 2/12 in Credit Card, Cellphone, and Headphones, and 3/12 in Camera.
It also produces non-zero KS counts in Cellphone, Camera, and Headphones.
The improvement is still limited, but it shows that validation-guided prompt revision can move generated discussions closer to real Reddit discussions on several metrics.

\begin{wrapfigure}{r}{0.62\textwidth}
    \centering
    \vspace{-1em}
    \includegraphics[width=0.60\textwidth]{figures/dotplot.png}
    \caption{
    Group-level baseline discrepancies relative to real-vs.-real variation.
    For each model and metric group, we divide the generated-vs.-real statistic by the repeated real-vs.-real median reference $R$.
    The left panel shows the $W_1$ ratio, and the right panel shows the $|\delta_{\mathrm{Cliff}}|$ ratio.
    The dashed vertical line marks the real-vs.-real reference at 1.0.
    Values closer to 1 indicate closer agreement with normal real-vs.-real variation.
    }
    \label{fig:group_level_baseline_discrepancy}
    \vspace{-1em}
\end{wrapfigure}

Figure~\ref{fig:group_level_baseline_discrepancy} shows the size of these gaps.
A ratio of 1 means that the generated-vs.-real gap is similar to the natural gap between two real-data samples.
Most ratios are above 1, often by a large margin.
This means that the mismatch is not only statistically significant, but also larger than normal real-vs.-real variation.
The largest gaps appear in Repetition/Semantic and Structure metrics, showing that generated discussions differ strongly from real discussions in semantic diversity and thread organization.
Narrative metrics also remain above the reference line.
Toxicity/Aggression is usually closer to the reference, but it is still not fully matched.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.88\textwidth]{figures/three_method_w1_cliff_alignment_radars_compact.png}
    \caption{
    Alignment comparison across OASIS, SynthPAI, and prompt-based calibration.
    The left radar plot shows Wasserstein alignment, and the right radar plot shows $|\delta_{\mathrm{Cliff}}|$ alignment across metric groups.
    Larger values indicate better alignment with real-vs.-real variation.
    Prompt-based calibration improves alignment over OASIS on several groups, especially for Wasserstein-based alignment, while the remaining gaps show that prompt revision does not fully solve the simulation-vs.-real mismatch.
    }
    \label{fig:calibration_radar}
\end{figure}

Figure~\ref{fig:calibration_radar} compares OASIS, SynthPAI, and prompt-based calibration using group-level alignment scores.
The radar plots show a different view from the p-value table.
Instead of only asking whether a metric is statistically distinguishable, they show how close each method is to the repeated real-vs.-real reference.
Prompt-based calibration improves the Wasserstein alignment over OASIS for several metric groups, especially Diversity/Semantic, Storyness, Toxicity/Aggression, and Structure.
This means that the calibrated generations move closer to the real-discussion distributions in terms of distance.
The $|\delta_{\mathrm{Cliff}}|$ alignment also improves over OASIS in several groups, although SynthPAI remains stronger on some groups such as Storyness and Structure.

Overall, the results show two main findings.
First, current simulators remain clearly distinguishable from real Reddit discussions, especially under the KS test.
Second, prompt-based calibration provides modest but useful improvement without changing the underlying model, adding fine-tuning, or using extra supervised training.
This supports our main claim: ThreadBench can reveal where simulators fail and can also measure whether calibration methods reduce the distributional gap.

\subsection{Ablation Study}
\label{sec:ablation}
K=1, 2, 3
add other baseline for k=3 to show that we also have better k=3 when other tries 

\subsection{Qualitative Observations}
\label{sec:observations}

Based on the generated discussions and their metric scores, we identify several qualitative patterns that help explain the distributional gaps measured by ThreadBench.

\ync{topcis and discussions could be expend: different thing but same way they talk, if persona helps, topic drift diversely in real in different domains(social drift more), use sft/RL agents to generate, consine cluster map for different models comapre to real}

\begin{wrapfigure}{r}{0.46\textwidth}
    \centering
    \vspace{-1em}
    \includegraphics[width=0.46\textwidth]{figures/real_generated_word_count_only.png}
    \caption{
    Word-count distribution for the real and generated Reddit comments shown in Appendix~\ref{app:discussion_examples}.
    Each point is one comment.
    Generated comments are generally longer and more concentrated in length, while real comments show a wider range from short reactions to longer personal recommendations.
    }
    \label{fig:example_word_count_distribution}
    \vspace{-1em}
\end{wrapfigure}

\textbf{Generated comments are more consistently helpful and length-aligned.}
As detailed in Appendix~\ref{app:discussion_examples}, LLM-generated users tend to answer in a polished and helpful style.
In the generated credit-card thread, many replies follow a similar template: recognize the user's budget concern, compare the Apple Card with the American Express Platinum Card, explain the annual-fee trade-off, and suggest a safer rewards strategy.
This makes individual comments look useful, but it also makes the overall thread more uniform.
As shown in Figure~\ref{fig:example_word_count_distribution}, generated comments are generally longer and more concentrated in length, whereas real Reddit comments vary more sharply, ranging from short reactions to longer personal recommendations.
This example-level pattern is consistent with the repeated real-vs.-real analysis in Figure~\ref{fig:repeated_sampling_w1} and Figure~\ref{fig:repeated_sampling_cliff}.
Real threads vary in what users say, how long comments become, and how reply trees develop.

\textbf{Generated discussions show high semantic overlap.}
Although generated comments are phrased differently, they often repeat the same core message.
In the simulated credit-card thread in Appendix~\ref{app:generated_discussion_example}, many agents say that the American Express Platinum Card has useful perks, but its annual fee is difficult to justify for a budget-conscious college student unless the user travels often and can use the benefits.
Most replies therefore recommend staying with the Apple Card, using cash-back rewards, or considering no-annual-fee alternatives.
The thread appears to contain many participants, but many comments restate the same advice in different words.
In contrast, the real Reddit examples in Appendix~\ref{app:real_discussion_example} are more context-specific.
Users discuss Canadian card availability, Aeroplan changes, Chase eligibility, purchase protection claims, card timing, and alternative card choices.
They also include short reactions and follow-up questions.
This creates a more uneven and semantically diverse discussion pattern.

\textbf{Generated users sound generally informed, while real users rely more on local context.}
The generated agents usually speak from a broad comparison view.
They give balanced financial advice and cover common factors such as annual fees, rewards, travel perks, and student budgets.
Real Reddit users contribute more partial and situated knowledge.
Some users only answer one eligibility issue, some mention one specific card, some describe a personal timing decision, and others ask narrow follow-up questions.
These comments are less polished on their own, but together they create a more varied thread. Generated discussions are readable, but they are often too uniformly helpful, too centered on the same advice, and too broad in their knowledge.
ThreadBench captures these gaps through metrics related to semantic uniformity, length variation, narrative content, and reply-tree structure.

==> sections/results-ablation.tex <==
% No table colours: boldface alone marks a passing metric.

\begin{table}[t]
\centering
\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.05}
\caption{%
  Draft budget $K$ against ThreadBench pass rate, per domain. Each   entry is the percentage of the twelve metrics indistinguishable   from held-out real threads, for the best backbone that ran every   $K$ with its planner and writer held fixed.}
\label{tab:ablation_k}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Domain} & $K{=}1$ & $K{=}2$ & $K{=}3$ & $\Delta$ (pp) \\
\midrule
Celebrity & 33\% (4/12) & 75\% (9/12) & \textbf{100\% (12/12)} & $+$67 \\
Game & 50\% (6/12) & 67\% (8/12) & \textbf{67\% (8/12)} & $+$17 \\
Movies & 50\% (6/12) & 83\% (10/12) & \textbf{92\% (11/12)} & $+$42 \\
News & 25\% (3/12) & 50\% (6/12) & \textbf{75\% (9/12)} & $+$50 \\
TV Series & 58\% (7/12) & 58\% (7/12) & \textbf{83\% (10/12)} & $+$25 \\
\midrule
\textit{Mean} & 43.3\% & 66.7\% & \textbf{83.3\%} & $+$40.0 \\
\bottomrule
\end{tabular}
\end{table}
